Finding large induced sparse subgraphs in $C_{>t}$-free graphs in quasipolynomial time

For an integer $t$, a graph $G$ is called {\em{$C_{>t}$-free}} if $G$ does not contain any induced cycle on more than~$t$ vertices. We prove the following statement: for every pair of integers $d$ and $t$ and a CMSO$_2$ statement~$\phi$, there exists an algorithm that, given an $n$-vertex $C_{>t}$-free graph $G$ with weights on vertices, finds in time $n^{O(\log^4 n)}$ a maximum-weight vertex subset $S$ such that $G[S]$ has degeneracy at most $d$ and satisfies $\phi$. The running time can be improved to $n^{O(\log^2 n)}$ assuming $G$ is $P_t$-free, that is, $G$ does not contain an induced path on $t$ vertices. This expands the recent results of the authors [to appear at FOCS 2020 and SOSA 2021] on the {\sc{Maximum Weight Independent Set}} problem on $P_t$-free graphs in two directions: by encompassing the more general setting of $C_{>t}$-free graphs, and by being applicable to a much wider variety of problems, such as {\sc{Maximum Weight Induced Forest}} or {\sc{Maximum Weight Induced Planar Graph}}.

==> automata.tex <==
\subsection{Automata}

In this section we present basic results on connections between \mso-definability of properties of graphs and recognizability using finite automata working on treedepth decompositions.
% Particularly, we mean one notion of decomposition: treedepth decompositions aka elimination forests.
The design of automata follows standard constructions that were developed in the 90s, see the monograph of Courcelle and Engelfriet for an introduction to the topic~\cite{CourcelleE12}.

For a finite alphabet $\Sigma$, a {\em{$\Sigma$-labelled forest}} is a (rooted, unordered) forest $F$
where every vertex $x\in V(F)$ is labelled with an element $\lbl(x)\in\Sigma$.
We assume that $\Sigma$-labelled forests are encoded as relational structures in a standard way using one binary parent relation
and one unary relation for each symbol in $\Sigma$.
Thus, when speaking about \mso formulas over $\Sigma$-labelled forest, we mean \mso formulas working over structures as above.

We will now show that \mso over labelled forests is equivalent to an automata model that we call {\em{threshold automata}}. To define them, we need the following notions. We use notation $\lmset\cdot\rmset$ for defining multisets. For a multiset $X$ and $\tau\in \N$, let $X\wedge \tau$ be the multiset obtained from $X$ by reducing the multiplicity of every element down to $\tau$, provided its multiplicity is larger than $\tau$. For a set $Q$ and $\tau\in \N$, by $\Multi(Q,\tau)$ we denote the family of all multisets with elements from $Q$, where each element appears at most $\tau$ times. Note that $|\Multi(Q,\tau)|=(\tau+1)^{|Q|}$.

\begin{definition}
 A {\em{threshold automaton}} is a tuple $\Aa=(Q,\Sigma,\tau,\delta,C)$, where:
 \begin{itemize}[nosep]
  \item $Q$ is a finite set of states;
  \item $\Sigma$ is a finite alphabet;
  \item $\tau\in \N$ is a nonnegative integer called the {\em{threshold}};
  \item $\delta\colon \Sigma\times \Multi(Q,\tau)\to Q$ is the transition function; and
  \item $C\subseteq \Multi(Q,\tau)$ is the accepting condition.
 \end{itemize}
 For a $\Sigma$-labelled forest $F$, the {\em{run}} of $\Aa$ on $F$ is the unique labelling $\xi\colon V(F)\to Q$ satisfying the following property for each $x\in V(F)$:
 $$\xi(x)=\delta(\lbl(x),\lmset\xi(y)\colon y\textrm{ is a child of }x\rmset\wedge \tau).$$
 We say that $\Aa$ {\em{accepts}} $F$ if 
 $$\lmset\xi(z)\colon z\textrm{ is a root of }F\rmset\wedge \tau \in C,$$
 where $\xi$ is the run of $\Aa$ on $F$.
\end{definition}

The proof of the following lemma is completely standard, hence we only provide a sketch.

\begin{lemma}\label{lem:mso-threshold}
 Let $\Sigma$ be a finite alphabet. Then for every sentence $\varphi$ of \mso over $\Sigma$-labelled forests there exists a threshold automaton $\Aa_\varphi$ working over $\Sigma$-labelled forests such that for every $\Sigma$-labelled forest $F$,
 $$F\models \varphi \qquad\textrm{if and only if}\qquad \Aa_\varphi\textrm{ accepts }F.$$
\end{lemma}
\begin{proof}[Sketch]
Let $q$ be the quantifier rank of $\varphi$, that is, the maximum number of nested quantifiers in~$\varphi$. It is well-known that there is only a finite number of pairwise non-equivalent \mso sentences over $\Sigma$-labelled forests with quantifier rank at most $q$. Let then $\Tp^q$ be the set containing one such sentence from each equivalence class. Then $\Tp^q$ is finite and we may assume that $\varphi\in \Tp^q$.

Consider a $\Sigma$-labelled forest $F$.
For a vertex $x\in V(F)$, let $F_x$ be the subtree of $F$ induced by $x$ and all its descendants. With $F_x$ we may associate its {\em{$q$-type}} defined as the set of all sentences from $\Tp^q$ satisfied in $F_x$, that is,
$$\tp^q(F_x)\coloneqq \{\,\psi\in \Tp^q\ \mid\ F_x\models \psi\,\}.$$
A standard argument using Ehrenfeucht-Fra\"isse games shows that $\tp^q(F_x)$ is uniquely determined by $\lbl(x)$ and the multiset $\lmset\tp^q(F_y)\colon y\textrm{ is a child of }x\rmset\wedge q$. Similarly, the type $\tp^q(F)$, defined analogously as above, is uniquely determined by the multiset $\lmset\tp^q(F_r)\colon r\textrm{ is a root of }F\rmset\wedge q$. This means that we may define a threshold automaton $\Aa_\varphi$ with state set $\Tp^q$ and threshold $q$ so that $\Aa_\varphi$ accepts $F$ if and only if $\varphi\in \tp^q(F)$, which is equivalent to $F\models\varphi$.
\end{proof}

For an integer $d$ and a finite alphabet $\Sigma_d$, a \emph{$(d,\Sigma_d)$-labeller} is a polynomial-time algorithm $\Lambda$ 
that, given a graph $G$ with a treedepth decomposition $F$
of depth at most $d$, computes a labelling $\Lambda[G,F] : V(G) \to \Sigma_d$ such that for every $v \in V(G)$, the label $\Lambda[G,F](v)$
depends only on the path from $v$ to the root in $F$ and the subgraph of $G$ induced by the vertices of the said path. 

\begin{lemma}\label{lem:mso}
 Let $d\in \N$ and let $\varphi$ be a sentence of \msotwo on graphs. There exists a finite alphabet $\Sigma_d$ and a $(d,\Sigma_d)$-labeller $\Lambda$, depending only on $d$, and a threshold automaton $\Aa_{\varphi,d}$ working over $\Sigma_d$-labelled graphs forests such that the following holds. For every graph $G$ and its treedepth decomposition $F$ of depth at most $d$
 $$G\models \varphi \qquad\textrm{if and only if}\qquad \Aa_{\varphi,d}\textrm{ accepts }(F,\Lambda[G,F]).$$
\end{lemma}

\begin{proof}
 We let $\Sigma_d=\{1,\ldots,d\}\times \{0,1\}^{\{1,\ldots,d\}}$, where the second coordinate of each element is treated as a function from $\{1,\ldots,d\}$ to $\{0,1\}$; note that $|\Sigma_d|=d\cdot 2^d$.
 Consider a graph $G$ and its treedepth decomposition $F$ of depth at most $d$.
 
 We now define the $(d,\Sigma_d)$-labeller $\Lambda$. Consider any $x\in V(G)$. Let $h$ be the depth of $x$ in $F$ and let $f$ be the function from $\{1,\ldots,d\}$ to $\{0,1\}$ defined as follows: for $i\geq h$ we set $f(i)=0$, and for $i<h$ we set $f(i)=1$ if and only if $x$ is adjacent to the unique ancestor of $x$ that is at depth $i$. Then, we set
 $$\Lambda[G,F](x)\coloneqq (h,f).$$
 By endowing $G$ and $F$ with the labelling function $\Lambda[G,F]$, we respectively obtain a $\Sigma_d$-labelled graph $\wh{G}$ and a $\Sigma_d$-labelled forest $\wh{F}$.
 Note that $\wh{G}$ can be computed from $G$ and $F$ in polynomial time.
 
 We now translate the sentence $\varphi$ as follows.
 
 \begin{claim}\label{cl:encoding}
  There is a sentence $\wh{\varphi}$ of \mso over $\Sigma_d$-labelled forests, which depends only on $\varphi$ and $d$, such that
  $$G\models \varphi \qquad\textrm{if and only if}\qquad \wh{F}\models \wh{\varphi}.$$
 \end{claim}
 \begin{claimproof}
 We obtain $\wh{\varphi}$ from $\varphi$ by a syntactic transformation as follows:
 \begin{itemize}
  \item For every quantification over an edge $e$, replace it with a quantification over the pair $x,y$ of its endpoints, followed by a check that $x$ and $y$ are indeed adjacent. Since the depth of $F$ is at most~$d$, which is a constant, this check can be performed using a first-order formula as follows: verify that $x$ and $y$ are in the ancestor-descendant relation in $\wh{F}$, retrieve the depth of $x$ and $y$ in $\wh{F}$ from their labels, and check that the label of the deeper of those two nodes contains information that the shallower one is adjacent.
  \item Replace each atom $\inc(z,e)$ with a disjunction checking that $z$ is among the endpoints of~$e$.  
  \item For every quantification over an edge set, say $\exists\,Y$, replace it with quantification of the form $\exists\,Y_1\ \exists\,Y_2\ \ldots\ \exists\,Y_{d-1}$, where $Y_i$ is interpreted as the set of all the deeper endpoints of those edges from~$Y$, whose shallower endpoint is at depth $i$. This quantification is followed by checking that for each $x\in Y_i$, indeed $x$ is adjacent to its unique ancestor at depth $i$, which is encoded in the label of $x$.
  \item Replace each atom $e\in Y$, where $e$ is an edge variable and $Y$ is an edge set variable, with a disjunction over $i\in \{1,\ldots,d\}$ of the following checks: denoting the endpoints of $e$ by $x$ and $y$, either $x$ is at depth $i$ and $y\in Y_i$, or vice~versa.
 \end{itemize}
 It is straightforward to see that $\wh{\varphi}$ obtained in this way satisfies the required property.
 \end{claimproof}

 By Lemma~\ref{lem:mso-threshold} and Claim~\ref{cl:encoding}, there exists a threshold automaton $\Aa$ such that $G\models \varphi$ if and only if $\Aa$ accepts $\wh{F}$. This finishes the proof.
\end{proof}


==> ptfree.tex <==
In this section we prove Theorem~\ref{thm:ptfree-mso}.

\subsection{Treedepth decompositions}

A \emph{treedepth decomposition} (sometimes also called an \emph{elimination forest}) of a graph $G$ is a rooted forest $F$
with $V(F) = V(G)$ and the following property: for every $uv \in E(G)$, $u$ and $v$ are in ancestor-descendant relation in $F$.
The \emph{depth} of a decomposition $F$ is the maximum number of vertices on a root-to-leaf path in $F$.
The \emph{treedepth} of a graph is the minimum possible depth of its treedepth decomposition.

In what follows all forests are rooted, so we drop the qualifier ``rooted''. 
Given a forest $F$ and $v \in V(F)$, by
$\parent_F(v)$ we denote the parent of $v$ (or $\parent_F(v) = \bot$ if $v$ is a root
    of a tree in $F$)
and by $\children_F(v)$ we denote the set of children of $v$ in $F$. 
The \emph{depth} of a vertex $v$ in a forest $F$, denoted by $\depth_F(v)$, is the number of vertices on the path
from $v$ to a root in $F$.
The subscript $F$ can be omitted if it is clear from the context.

A treedepth decomposition $F$ of $G$ 
is \emph{proper} if for every $u \in V(G)$ with $v = \parent_F(u) \neq \bot$
there exists a descendant $w$ of $u$ in $F$ (possibly $w = u$) with
$vw \in E(G)$. 
It is easy to observe that any treedepth decomposition can be turned into a proper one
without increasing its depth: interatively, if a pair $(u,v)$ violates the definition of a proper
treedepth decomposition, reattach $u$ to be a child of $\parent_F(v)$
(or a separate root if $\parent_F(v) = \bot$);
this iterative process ends after a polynomial number of steps as each step strictly decreases
the sum of the depths of all vertices.

The following observation is also immediate.
\begin{lemma}\label{lem:proper-td}
Let $G$ be a graph, $F$ a proper treedepth decomposition of $G$, and $F'$ be a subgraph of $F$ closed under taking parents.
Then the family of vertex sets of connected components of $G-V(F')$ is exactly the same as the family of vertex sets 
of connected components of $F-V(F')$. 
\end{lemma}

We need the following result.
\begin{lemma}[\cite{AtminasLR12}]\label{lem:ALR}
For every integers $a$ and $b$ there exists an integer $\ALR(a,b)$, such 
that if $G$ contains a path with $\ALR(a,b)$ vertices,
then $G$ contains either $K_{b,b}$ as a subgraph 
or a path on $a$ vertices as an induced subgraph.
\end{lemma}
\begin{corollary}\label{cor:ALR}
For every integers $t$ and $k$ there exists an integer $\TD(t,k)$
such that if $G$ is $P_t$-free and of treewidth less than $k$,
     then the treedepth of $G$ is bounded by $\TD(t,k)$.
\end{corollary}
\begin{proof}
Since $K_{k+1,k+1}$ is of treewidth $k$, 
      $G$ does not contain $K_{k+1,k+1}$ as a subgraph.
By Lemma~\ref{lem:ALR}, $G$ does not contain a path
on $\ALR(t, k+1)$ vertices as a subgraph. 
As a depth-first search tree is a treedepth decomposition of a connected graph
and every path in a depth-first search tree of $G$ is a path in $G$,
the treedepth of $G$ is less than $\ALR(t,k+1)$.
Hence, we can set $\TD(t,k) = \ALR(t, k+1) - 1$.
\end{proof}

\input{automata}

\subsection{From treewidth to treedepth}

By Lemma~\ref{lem:mso-threshold} and Corollary~\ref{cor:ALR}, to prove Theorem~\ref{thm:ptfree-mso}
it suffices to prove the following statement.
\begin{theorem}\label{thm:td-ptfree-mso}
For every fixed constants $d,t$,
a threshold automaton $\Aa = (Q,\Sigma,\tau,\delta,C)$,
and a $(d,\Sigma)$-labeller $\Lambda$,
there exists an algorithm that
given an $n$-vertex $P_t$-free graph $G$ with vertex weights $\wei : V(G) \to \mathbb{N}$,
in time $n^{\Oh(\log^2 n)}$ finds a subset $A \subseteq V(G)$
and a treedepth decomposition $F$ of $G[A]$ of depth at most $d$
such that $\Aa$ accepts $(F, \Lambda[G[A],F])$
and the weight of $A$ is at least the maximum possible
weight of a set $A_0 \subseteq V(G)$ such that
there exists a \emph{proper} treedepth decomposition $F_0$
of $G[A_0]$ of depth at most $d$ such that $\Aa$ accepts $(F_0,\Lambda[G[A_0], F_0])$.
\end{theorem}

Let us formally verify that Theorem~\ref{thm:td-ptfree-mso} implies Theorem~\ref{thm:ptfree-mso}.
\begin{proof}[Proof of Theorem~\ref{thm:ptfree-mso}]
Let $\phi_{\tw < k}$ be an \msotwo sentence promised
by Lemma~\ref{lem:mso-tw-formula}, that is, $G \models \phi_{\tw < k}$ 
if and only if the treewidth of $G$
is less than $k$.

Let $d = \TD(t,k)$ where $\TD$ comes from Corollary~\ref{cor:ALR}. 
Apply Lemma~\ref{lem:mso} to $d$ and a sentence $\varphi' := \varphi \wedge \phi_{\tw < k}$, 
obtaining an alphabet $\Sigma_d$, a $(d,\Sigma_d)$-labeller $\Lambda$
and a threshold automaton $\Aa_{\varphi', d}$ working over $\Sigma_d$-labelled 
forests. 
We have that for every $A \subseteq V(G)$, $G[A]$ is of treewidth less than $k$
and $G[A] \models \varphi$ if and only if for every treedepth decomposition $F$ of $G[A]$
of depth at most $d$, $\mathcal{A}_{\varphi', d}$ accepts $(F, \Lambda[G[A],F])$. 
Furthermore, the choice of $d$ implies that for every $G[A]$ that is of treewidth less than $k$,
  there exists a treedepth decomposition of $G[A]$ of depth at most $d$.

Hence, we can apply the algorithm of Theorem~\ref{thm:td-ptfree-mso}
to the graph $G$ with vertex weights $\wei$, threshold automaton $\Aa_{\varphi',d}$
and $(d,\Sigma_d)$-labeller $\Lambda$, obtaining a pair $(A,F)$, and return the set $A$.
\end{proof}

\subsection{Heavy vertex}

In our branching algorithm for Theorem~\ref{thm:ptfree-mso}, we will follow the same choice of a branching pivot as in~\cite{PPR20SODA}. Let $G$ be a graph. For every unordered pair $\{u,v\} \in \binom{V(G)}{2}$,
the \emph{bucket} $\Bb^G_{u,v}$ consists of all induced paths in $G$
with endpoints $u$ and $v$. Clearly, $\Bb^G_{u,v}$ is nonempty if and only if
$u$ and $v$ are in the same connected component.

Fix $\varepsilon > 0$. A vertex $w \in V(G)$ is \emph{$\varepsilon$-heavy}
if for at least $\varepsilon \binom{|V(G)|}{2}$ pairs $\{u,v\} \in \binom{V(G)}{2}$
it holds that 
$$|\{P \in \Bb^G_{u,v}~|~N[w] \cap V(P) \neq \emptyset\}| > \varepsilon |\Bb^G_{u,v}|.$$
We will use the following lemma of~\cite{PPR20SOSA}:
\begin{lemma}\label{lem:heavy}
For every $t \geq 2$, a connected nonempty $P_t$-free graph contains 
a $\frac{1}{2t}$-heavy vertex.
\end{lemma}
Since a $P_t$-free graph contains $\Oh(n^{t-1})$ induced paths, one can enumerate
all buckets $\Bb^G_{u,v}$ in polynomial time and hence detect a heavy vertex
promised by Lemma~\ref{lem:heavy} in polynomial time. 

\subsection{Branching algorithm}

The algorithm of Theorem~\ref{thm:td-ptfree-mso} is a branching algorithm
that explores the space of possible outputs $(A,F)$ so that the recursion tree has size $n^{\Oh(\log^2 n)}$. 
Note that we treat $d$, $t$, and all ingredients of $\Aa$ as constants.

Let us fix a pair $(A_0,F_0)$ such that $F_0$ is a proper treedepth
decomposition of $G[A_0]$ of depth at most $d$, $\Aa$ accepts $(F_0, \Lambda[G[A_0], F_0])$,
and the weight of $A_0$ is maximum possible.
Let $\xi_0$ be the run of $\Aa$ on $(F_0, \Lambda[G[A_0], F_0])$. 

\paragraph{Partial solutions.}
Our recursive algorithm proceeds by constructing larger and larger partial solutions.
\begin{definition}
A \emph{partial solution} $\psol$ consists of:
\begin{enumerate}
\item Two disjoint vertex sets $\VtxTaken^\psol, \VtxDeleted^\psol \subseteq V(G)$;
 we additionally denote
 $\VtxFree^\psol := V(G) \setminus (\VtxTaken^\psol \cup \VtxDeleted^\psol)$.
\item A treedepth decomposition $F^\psol$ of $G[\VtxTaken^\psol]$ of depth at most $d$;
we additionally 
define a labelling $\lambda^\psol : \VtxTaken^\psol \to \Sigma$
that assigns to $v \in \VtxTaken^\psol$
a label $\lambda^\psol(v) = \Lambda[G[\VtxTaken^\psol], F](v)$. 
\item A multiset $M^\psol \in \Multi(Q,\tau)$ and multisets
$M_v^\psol \in \Multi(Q,\tau)$ for every $v \in \VtxTaken^\psol$;
we additionaly define $q_v^\psol := \delta(\lambda^\psol(v), M_v^\psol)$ for every $v \in \VtxTaken^\psol$
and require that the following holds:
\begin{itemize}
\item $M^\psol \in C$, 
\item 
$M^\psol = \lmset q_v^\psol~|~\parent_{F^\psol}(v) = \bot\rmset \wedge \tau.$
\item 
For every $v \in \VtxTaken^\psol$ we have
$M_v^\psol = \lmset q_w^\psol~|~w \in \children_{F^\psol}(v) \rmset \wedge \tau$.
\end{itemize}
\end{enumerate}
For all notation above, we allow omitting
the superscript $\psol$ if it is clear from the context. 
\end{definition}

The intuitive meaning of a partial solution $\psol = (\VtxTaken, \VtxDeleted, F, M, (M_v)_{v \in \VtxTaken})$ is as follows.
The sets $\VtxTaken$ and $\VtxDeleted$ are vertices that were already decided to be taken and not taken, respectively, to the solution $A_0$, i.e., we aim at
 $\VtxTaken \subseteq A_0$ and $\VtxDeleted \cap A_0 = \emptyset$. 
The forest $F$ is meant as the restriction of the sought treedepth decomposition $F_0$ of $G[A_0]$
to set $\VtxTaken$. 
We require that whenever $v \in \VtxTaken$, then also all ancestors of $v$ in $F_0$
are in $\VtxTaken$ (and hence in $F$). That is, we want $F$ to be a subgraph of $F_0$ closed
under taking parents.
The assumption that the labeller $\Lambda$ assigns a label on a vertex $v$
that only depends on the path from $v$ upwards in $F_0$ and the subgraph of $G$
induced by the vertices of the said path implies that we can hope for
$\lambda^\psol(v) = \Lambda[G[A_0], F_0](v)$ for every $v \in \VtxTaken$. 

We expect that $q_v = \xi_0(v)$ for every $v \in \VtxTaken$.
Consequently, we expect that
$M = \lmset\xi_0(v)~|~\parent_{F_0}(v) = \bot\rmset \wedge \tau$
and that for every $v \in \VtxTaken$ it holds that
$M_v = \lmset\xi_0(w)~|~\parent_{F_0}(w) = v\rmset \wedge \tau$. 
In particular, we require that for every $q \in Q$, the number of
tree roots $v$ of $F$ with $q_v = q$ equals exactly the multiplicity of $q$
in $M$, with the exception that if $q$ appears $\tau$ times in $M$, we allow more such
roots in $F$. 
Similarly, for every $v \in \VtxTaken$ and every $q \in Q$,
the number of children $w$ of $v$ in $F$ with $q_w = q$ should equal exaclty the multiplicity
of $q$ in $M_v$, again with the exception that if $q$ appears $\tau$ times in $M_v$,
we allow more such children in $F$.

The above intutition allows the following definitions.
\begin{definition}
A partial solution $\psol$ is \emph{lucky} if 
$\VtxTaken^{\psol} \subseteq A_0$,
$\VtxDeleted^\psol \cap A_0 = \emptyset$,
$F^\psol$ is a subtree of $F_0$ closed under taking parents,
  and $q^\psol_v = \xi_0(v)$
%$M^\psol = \lmset\xi_0(w)~|~w \in A_0 \wedge \parent_{F_0}(w) = \bot\rmset \wedge \tau$,
%and
%$M_v^{\psol} = \lmset\xi_0(w)~|~w \in \children_{F_0}(v)\rmset \wedge \tau$
for every $ v \in \VtxTaken^{\psol}$.
\end{definition}

\begin{definition}
A partial solution $\psol_2$ \emph{extends} partial solution $\psol_1$
if 
\begin{itemize}
\item $\VtxTaken^{\psol_1} \subseteq \VtxTaken^{\psol_2}$ 
and $\VtxDeleted^{\psol_1} \subseteq \VtxDeleted^{\psol_2}$ (and hence
 $\VtxFree^{\psol_1} \supseteq \VtxFree^{\psol_2}$).
\item $F^{\psol_1}$ is a subgraph of $F^{\psol_2}$ closed under taking parents.
\item $M^{\psol_1} = M^{\psol_2}$ and $M_v^{\psol_1} = M_v^{\psol_2}$ for every
$v \in \VtxTaken^{\psol_1}$. 
\end{itemize}
Furthermore, for a set $D \subseteq \VtxTaken^{\psol_1}$, we say that
$\psol_2$ \emph{extends $\psol_1$ into $D$} if
$\VtxFree^{\psol_1} \setminus \VtxFree^{\psol_2} \subseteq D$ 
and 
$\psol_2$ \emph{extends $\psol_1$ completely into $D$} if
$\VtxFree^{\psol_1} \setminus \VtxFree^{\psol_2} = D$. 
\end{definition}

The following observation is straightforward from the definition of a run and partial solution:
\begin{lemma}\label{lem:psol2sol}
If $\psol$ is a partial solution, then $F^\psol$ is a treedepth
decomposition of $G[\VtxTaken^\psol]$ of depth at most $d$ and $\Aa$ accepts
$(F^\psol, \Lambda[G[\VtxTaken^\psol], F^\psol])$. 
\end{lemma}
The above lemma allows to define a \emph{weight} of a partial solution $\psol$
to be the weight of $\VtxTaken^\psol$.

A partial solution $\psol$ is \emph{final} if $\VtxFree^\psol = \emptyset$.
Since for every partial solution $\psol$, 
the tuple $(\VtxTaken^\psol, \VtxDeleted^\psol \cup \VtxFree^\psol, F^\psol, M^\psol, (M_v^\psol)_{v\in \VtxTaken^\psol})$ is also a partial solution that is final and of the same weight as $\psol$,
our task is to find a final partial solution of weight at least the weight of $A_0$.

\paragraph{Cleanup step.}
To design the algorithm, we will need a simple cleanup phase, based on the following observation.
\begin{lemma}\label{lem:cleanup}
Assume $\psol$ is a lucky partial solution and $v \in \VtxFree^\psol$
is such that $N_G(v) \cap \VtxTaken^\psol$ contains a vertex of depth $d$
in $F^\psol$ or two vertices that are not in ancestor-descendant relationship in $F^\psol$.
Then, $v \notin A_0$.
\end{lemma}
\begin{proof}
Since $\psol$ is lucky, $F^\psol$ is a subgraph of $F_0$ closed under taking parents.
Then, $v \in A_0$ would contradict the assumption that $F_0$ is a treedepth decomposition
of $G[A_0]$ of depth at most $d$.
\end{proof}
For a partial solution $\psol$ and a set $D \subseteq \VtxFree^\psol$, 
a \emph{cleaning operation} of $(\psol,D)$ constructs
a partial solution $\psol'$ extending $\psol$ into $D$ by putting all vertices $v \in D$
that satisfy the assumptions of Lemma~\ref{lem:cleanup} into $\VtxDeleted^{\psol'}$. 
Lemma~\ref{lem:cleanup} asserts that if $\psol$ is lucky, so is $\psol'$. 

\paragraph{Splitting into connected components.}
To treat independently connected components of $G[\VtxFree^\psol]$ for a partial solution $\psol$,
we need the following
observation that follows immediately from the requirement
on $\VtxTaken^\psol$ being closed under taking parents in $F^\psol$ and some amount of symbol pushing.
\begin{lemma}\label{lem:psol-assemble-comps}
Let $\psol$ be a partial solution and let $D$ be a connected component of $G[\VtxFree^\psol]$. 
Let $\psol'$ be a partial solution that extends $\psol$ into $D$.
Let $D_1,\ldots,D_\ell$ be the connected components of $G[D \cap \VtxFree^{\psol'}]$
and let $\psol_i$ be a partial solution that extends $\psol'$ completely into $D_i$. 

Define a partial solution $\psol''$ as follows:
\begin{itemize}
\item $\VtxTaken^{\psol''} = \bigcup_{i=1}^\ell \VtxTaken^{\psol_i}$
and $\VtxDeleted^{\psol''} = \bigcup_{i=1}^\ell \VtxDeleted^{\psol_i}$.
\item $F^{\psol''} = \bigcup_{i=1}^\ell F^{\psol_i}$.
\item $M^{\psol''} = M^{\psol}$ (which is equal to $M^{\psol'}$ and every $M^{\psol_i}$, $1 \leq i \leq \ell$). 
\item $M_v^{\psol''} = M_v^{\psol'}$ if $v \in \VtxTaken^{\psol'}$ and
$M_v^{\psol''} = M_v^{\psol_i}$ if $v \in \VtxTaken^{\psol_i}$, $1 \leq i\leq \ell$.
\end{itemize}
Then $\psol''$ is a partial solution that extends $\psol$ completely into $D$
and extends $\psol'$ completely into $D \setminus \VtxTaken^{\psol'}$. 
Furthermore, 
$\wei(\psol'') = \wei(\psol') + \sum_{i=1}^\ell (\wei(\psol_i) - \wei(\psol'))$.
\end{lemma}
\begin{proof}
Apart from direct checks from the definitions, the only observation needed is that
$F^{\psol'}$ is a common closed under taking parents subforest of 
every $F^{\psol_i}$, $1 \leq i \leq \ell$, and the sets
$V(F^{\psol_i}) \setminus V(F^{\psol'})$ are pairwise disjoint.
Hence, $F^{\psol''} = \bigcup_{i=1}^\ell F^{\psol_i}$ is well-defined.
\end{proof}

\paragraph{Closures.}
To prove that our branching algorithm finds a good enough solution, 
we will need the following observation.

\begin{lemma}\label{lem:closure}
For every $v \in A_0$ 
there exists a subset $\closure_{A_0,F_0}(v) \subseteq A_0$
of size at most $d^2 (|Q|\tau)^{d-1}$ such that 
\begin{itemize}
\item $v \in \closure_{A_0,F_0}(v)$;
\item $\closure_{A_0,F_0}(v)$ is closed under taking parents; and
\item for every $u \in \closure_{A_0,F_0}(v)$ it holds that
\begin{equation}\label{eq:closure}
  \lmset\xi_0(w)~|~w \in \children_{F_0}(u)\rmset \wedge \tau = 
  \lmset\xi_0(w)~|~w \in \children_{F_0}(u) \cap \closure_{A_0,F_0}(v)\rmset \wedge \tau.
\end{equation}
\end{itemize}

Furthermore, assume that $\psol$ is a lucky partial solution,
$D$ is a connected component of $G[\VtxFree^\psol]$,
and $v \in D \cap A_0$. 
Then there exists a subset $\closure_{A_0,F_0}^\psol(v) \subseteq D \cap A_0$
of size at most $d^2 (|Q|\tau)^{d-1}$ such that 
$\VtxTaken^\psol \cup \closure_{A_0,F_0}^\psol(v)$ satisfies the requirements
for $\closure_{A_0,F_0}(v)$ itemized above.
\end{lemma}
\begin{proof}
For every $u \in A_0$ consider the following recursive definition of a set $C(u)$:
for every $q \in Q$,
let $D(u,q)$ be $\tau$ children of $u$ in $F_0$ from
$\{w \in \children_{F_0}(u)~|~\xi_0(w) = q\}$ (or all of them if there are
fewer than $\tau$ such children),
and define 
$C(u) = \{u\} \cup \bigcup_{q \in Q} \bigcup_{w \in D(u,q)} C(w)$.

For the first part, 
define $\closure_{A_0,F_0}(v)$ to be the union of all sets $C(u)$
for $u$ lying on a path from $v$ to a root in $F_0$.
For the second part,
define $\closure_{A_0,F_0}^\psol(v)$ to be the union of all sets $C(u)$
for $u$ lying on a path from $v$ upward in $F_0$ to a first vertex 
of $\VtxTaken^\psol$ (exclusive). 

To see that $\closure_{A_0,F_0}^\psol(v) \subseteq D$, recall that 
$F_0$ is a proper treedepth decomposition. Together with the assumption
that $\psol$ is lucky it implies that no edge of $F_0$ connects two vertices
of different connected components of $G[\VtxFree^\psol]$. 
Since $\closure_{A_0,F_0}^\psol(v)$ induces a subtree of $F_0$, 
we have $\closure_{A_0,F_0}^\psol(v) \subseteq D$

For the size bound, observe 
first that every set $D(u,q)$ is of size at most $|Q|\tau$.
Hence, by a straightforward bottom-up induction, 
if a vertex $u$ is at depth $j$ in $F_0$, then $C(u)$ is of size at most 
$\sum_{i=0}^{d-j} (|Q|\tau)^i$.
The size bound follows.

Other promised properties of $\closure_{A_0,F_0}(v)$ 
and $\closure_{A_0,F_0}^\psol(v)$ are immediate from the definitions.
\end{proof}

\paragraph{Setting of a recursive call.}
In a recursive call, the algorithm is given a partial solution $\psol$ and a component $D$ of $G[\VtxFree^\psol]$.
The algorithm outputs a partial solution $\psol'$ that extends $\psol$ completely into $D$.
Later in this section we will prove the following invariant:
\begin{lemma}\label{lem:prop-lucky}
If $\psol$ is lucky, then a recursive call applied to
$\psol$ and a component $D$ of $G[\VtxFree^\psol]$ outputs
a partial solution $\psol'$ that extends $\psol$ completely into $D$
and $\wei(\psol') - \wei(\psol) \geq \wei(A_0 \cap D)$. 
\end{lemma}

\paragraph{Top level of the recursion.}
On top level, the algorithm starts by guessing $M \subseteq \Multi(Q,\tau)$
aiming at $M = \lmset\xi_0(w)~|~w\in A_0 \wedge \parent_{F_0}(w) = \bot\rmset \wedge \tau$
and, for every $q \in Q$,
guessing a set $C_q$ of $\tau$ vertices (or all of them, if there are fewer than $\tau$ such vertices)
$v \in A_0$ with $\xi_0(v) = q$ and $\parent_{F_0}(v) = \bot$.
Then, for every $q \in Q$ and $v \in C_q$, the algorithm guesses a set $\Gamma(v)$
of size at most $d^2 (|Q|\tau)^{d-1}$, aiming at $\Gamma(v) = \closure_{A_0,F_0}(v)$
where $\closure_{A_0,F_0}(v)$ is the set promised by Lemma~\ref{lem:closure}. 
Let $\VtxTaken = \bigcup_{q \in Q} \bigcup_{v \in C_q} \Gamma(v)$ and $\VtxDeleted = \emptyset$.
The algorithm guesses a forest $F$ with vertex set $\VtxTaken$.
For every $u \in \VtxTaken$, the algorithm guesses a set 
$M_u \subseteq \Multi(Q,\tau)$. 
Finally, with every generated tuple $\psol = (\VtxTaken, \VtxDeleted, F, M, (M_u)_{u \in \VtxTaken})$
that satisfies all the properties of a partial solution, the algorithm proceeds further as follows.

Let $D_1,D_2,\ldots,D_\ell$ be the connected components of
$G[\VtxFree^\psol]$. For every $1 \leq i \leq \ell$ the algorithm invokes a recursive call
on $\psol$ and $D_i$, obtaining a partial solution $\psol_i$ extending $\psol$ completely
into $D_i$, and uses Lemma~\ref{lem:psol-assemble-comps} (for $\psol'=\psol$)
to assemble a partial solution $\psol''$ extending $\psol$ completely into $\VtxFree^\psol$
(and thus $\psol''$ is final). 
The algorithm outputs the set pair $(\VtxTaken^{\psol''}, F^{\psol''})$ of maximum weight
over all enumerated partial solutions $\psol$. 

From the above discussion it follows that in at least one subcase the enumerated tuple $\psol$ will be a lucky partial solution.
Lemma~\ref{lem:prop-lucky} ensures that for a lucky $\psol$ the output weight
is at least the weight of $A_0$.

Since  $|Q|$, $\tau$, and $d$ are constants, 
there is a constant number of choices of $M$,
$n^{\Oh(1)}$ choices for all sets $C_q$,
$n^{\Oh(1)}$ choices for all sets $\Gamma(v)$,
and a constant number of choices for $F$ and all sets $M_u$.
Hence, we consider a polynomial number of subcases.

It remains to design the recursive algorithm
running within the promised time bound
so that Lemma~\ref{lem:prop-lucky} is satisfied.

\paragraph{Details of the recursive algorithm.}
Consider a recursive call with partial solution $\psol$ and 
a component $D$ of $G[\VtxFree^\psol]$. 
Let $v \in D$ be a vertex that is $\frac{1}{2t}$-heavy in $G[D]$ (cf. Lemma~\ref{lem:heavy}). 
We branch on $v$ as follows.
In a failure branch (guessing $v \notin A_0$), we define $\psol^\ast$ to be the partial solution $\psol$ with
additionally $v$ put into $\VtxDeleted^{\psol^\ast}$. 
In a success branch (guessing $v \in A_0$), we branch further as follows.
\begin{itemize}
\item 
We guess a set $\Gamma(v) \subseteq D$ of size at most $d^2 (|Q|\tau)^{d-1})$,
aiming at $\Gamma(v) = \closure_{A_0,F_0}^\psol(v)$ (cf. Lemma~\ref{lem:closure}).
\item 
For every choice of $\Gamma(v)$, 
we guess a forest $F^\ast$ of depth at most $d$ on vertex set $\VtxTaken^\psol \cup \Gamma(v)$
such that $F^\psol$ is a subforest of $F^\ast$ closed under taking parents.
\item Furthermore, we guess a set $M_u^\ast \subseteq \Multi(Q,\tau)$ for every $u \in \Gamma(v)$.
\end{itemize}
We define a tuple $\psol^\ast = (\VtxTaken^{\psol} \cup \Gamma(v), \VtxDeleted^{\psol}, F^\ast, M^\psol, (M_u^\psol)_{u \in \VtxTaken^{\psol}} \cup (M_u^\ast)_{u \in \Gamma(v)})$ and
if $\psol^\ast$ is a partial solution, we continue further with this branch. 
Note that there is one generated partial solution $\psol^\ast$ in the failure branch
and $n^{\Oh(1)}$ generated partial solutions $\psol^\ast$ in the success branch.

For every generated partial solution $\psol^\ast$ (including the one from the failure branch), 
let $\psol'$ be the result of cleaning $(\psol^\ast, D \cap \VtxFree^{\psol^\ast})$. 
Enumerate the connected components of $G[D \setminus \VtxTaken^{\psol'}]$ as
$D_1,\ldots,D_\ell$, and for every $1 \leq i \leq \ell$ apply the recusive call to 
$\psol'$ and $D_i$, obtaining a partial solution $\psol_i$ completely extending $\psol'$
into $D_i$. Use Lemma~\ref{lem:psol-assemble-comps} to obtain a solution
$\psol''$ completely extending $\psol'$ into $D \setminus \VtxTaken^{\psol'}$
and at the same time completely extending $\psol$ into $D$. 
Finally, output the partial solution $\psol''$ of maximum weight among all found.
This completes the description of the recursive call. 

We now prove Lemma~\ref{lem:prop-lucky}.
\begin{proof}[Proof of Lemma~\ref{lem:prop-lucky}.]
The proof proceeds by induction on the size of $D$ in the recursive call.

Consider a recursive call on $\psol$ and $D$ and assume that $\psol$ is lucky. 
If $v \notin A_0$, then $\psol^\ast$ in the failure branch is lucky.
Otherwise, by Lemma~\ref{lem:closure}, there exists  $\psol^\ast$ enumerated in the success branch
that is lucky. 
By Lemma~\ref{lem:cleanup}, the corresponding result $\psol'$ of cleaning is also lucky.
We infer that in all cases, there is an enumerated partial solution $\psol'$ that is lucky.

For the choice of $\psol'$ that is lucky, if $D_1,\ldots,D_\ell$
are the connected components of $G[D \setminus \VtxTaken^{\psol'}]$,
then for every $1 \leq i \leq \ell$ the inductive assumption implies that the returned solution $\psol_i$
satisfies $\wei(\psol_i) - \wei(\psol') \geq \wei(A_0 \cap D_i)$.
By Lemma~\ref{lem:psol-assemble-comps} we have $\wei(\psol'') - \wei(\psol) \geq \wei(A_0 \cap D)$, as desired.
\end{proof}

\paragraph{Running time bound.}
It remains to argue about the running time bound.
Note that in a recursive call for $\psol$ and $D$, every child subcall treats a component $D_i$
which is a proper subset of $D$ (as $v \in D \setminus D_i$). 
Thus, the depth of the recursion tree is bounded by $n$
and it suffices to argue that the recursion tree has $n^{\Oh(\log^2 n)}$ leaves.

The \emph{level} of the recursive call on $\psol$ and $D$ is $\lceil \log_2(|D|+1) \rceil$. 
Since $D \neq \emptyset$, every level is a positive integer bounded by $\log_2(n+1)$. 
Furthermore, the level of a child subcall is never higher than the level of a parent call.
Consequently, it suffices to argue that a subtree of the recursion tree consisting
of recursive calls of the same level $p$ has $n^{\Oh(\log n)}$ leaves.

Case $p=1$ corresponds to leaf recursive calls with $|D|=1$ and the claim is trivial.
Henceforth we assume $p > 1$ and thus the components $D$ in question have at least $2$ vertices.

Recall that every recursive call invokes one failure branch child subcall
and $n^{\Oh(1)}$ success branch child subcalls. 
To show that a subtree of the recursion tree consisting of recursive calls
of level $p$ has $n^{\Oh(\log n)}$ leaves it suffices to show that
any upwards path in the recursion tree visiting only recursive calls of the same level $p$
visits $\Oh(\log n)$ edges that corresponds to success branch child subcalls. 

Intuitively, the failure branch only progresses by deleting one vertex,
but a success branch leads to bigger progress due to the choice of a heavy vertex
as the branching pivot. 
To analyse this progress, we need a few notions.

Let $\psol$ be a partial solution. The \emph{depth cap} of a vertex $v \in \VtxFree^\psol$
is $\depthcap_\psol(v) := \max_{u \in N_G(v) \cap \VtxTaken^\psol} \depth_{F^\psol}(u)$;
we use the convention the maximization attains $0$ if it is made over an empty set
(that is, the depth cap of a vertex $v \in \VtxFree^\psol$
 with $N_G(v) \cap \VtxTaken^\psol = \emptyset$ 
 equals $0$).
Note that $\depthcap_\psol(v) \in \{0,1,\ldots,d\}$. 

Recall that for a graph $G'$ and a pair $\{u,v\} \in \binom{V(G')}{2}$,
a bucket $\Bb^{G'}_{u,v}$ constists of all induced paths with endpoints $u$ and $v$.
For a partial solution $\psol$ and a component $D$ of $G[\VtxFree^\psol]$,
we define the following two measures.
For every $\{u,v\} \in \binom{D}{2}$ we define
$$\bucketmeasure^{\psol,D}(\{u,v\}) = \sum_{P \in \Bb^{G[D]}_{u,v}} \sum_{w \in V(P)} 
  (d + 1- \depthcap_\psol(w)).$$
Aggregating the above, we define
$$\measure(\psol,D) = \sum_{\{u,v\} \in \binom{D}{2}} \log_2 \bucketmeasure^{\psol,D}(\{u,v\}).$$
Observe that, as $G$ is $P_t$-free, $1 \leq \bucketmeasure^{\psol,D}(\{u,v\}) \leq (d+1)(t-1)|D|^{t-1}$
for every $\{u,v\} \in \binom{D}{2}$
Consequently,
 \begin{equation}\label{eq:meas}
  0 \leq \measure(\psol,D) = \Oh(|D|^2 \log_2 |D|).
 \end{equation}

Consider now a recursive call with a partial solution $\psol$ and component $D$
of level $p > 1$. 
During the recursive call, the algorithm enumerates a family of partial solutions 
of polynomial size and, for every enumerated partial solution $\psol'$ and every 
$D'$ being a connected component
of $G[D \setminus \VtxTaken^{\psol'}]$, recurses on $\psol'$ and $D'$.
For  fixed $\psol'$, at most one component $D'$ satisfies $|D'| > |D|/2$. Hence,
for  fixed $\psol'$ there is at most one child call for $\psol'$ and a connected component $D'$
that is of level $p$. Furthermore, since $\VtxTaken^\psol \subsetneq \VtxTaken^{\psol'}$
and $D' \subsetneq D$, we have
that $\depthcap_{\psol'}(v) \geq \depthcap_\psol(v)$ for every $v \in D'$,
$\Bb^{G[D']}_{u,v} \subseteq \Bb^{G[D]}_{u,v}$ for every $\{u,v\} \in \binom{D'}{2}$
and, hence, $\measure(\psol',D') \leq \measure(\psol,D)$.

Together with~\eqref{eq:meas}, the following lemma proves that
any upwards path in the recursion tree visiting only recursive calls of the same level $p$
visits $\Oh(\log n)$ edges that corresponds to success branch child subcalls,
concluding the analysis of the running time bound and the proof of
Theorem~\ref{thm:td-ptfree-mso}.

\begin{lemma}\label{lem:meas}
Consider a recursive call on a partial solution $\psol$ and a component $D$ of level $p > 1$
and a child recursive call on a partial solution $\psol'$ and a component $D'$ of the same level $p$,
coming from the success branch.
Then for some universal constant $c$ it holds that
$$\measure(\psol,D) - \measure(\psol',D') \geq \frac{c}{t^3(d+1)} |D|^2$$
\end{lemma}
\begin{proof}
Let $v$ be the branching pivot used in the recursive call for $\psol$ and $D$.
Let $K \subseteq \binom{D}{2}$ be the family of those pairs $\{u_1,u_2\} \in \binom{D}{2}$
such that $N[v]$ intersects more than a $\frac{1}{2t}$ fraction of paths
of $\Bb^{G[D]}_{u_1,u_2}$. 
Recall that $v$ is $\frac{1}{2t}$-heavy and, hence, $|K| \geq \frac{1}{2t} \binom{D}{2}$.

Consider $\{u_1,u_2\} \in K \cap \binom{D'}{2}$ and $P \in \Bb^{G[D]}_{u_1,u_2}$
such that $V(P) \cap N[v] \neq \emptyset$.
Let $w \in V(P) \cap N[v]$. 
Note that $v \in \VtxTaken^{\psol'}$ as $\psol'$ comes from the success branch.
If $\depth_{F^{\psol'}}(v) \leq \depthcap_\psol(w)$
or $\depth_{F^{\psol'}}(v) = d$, then 
$w \in \VtxDeleted^{\psol'}$ as $w$ is moved to $\VtxDeleted^{\psol'}$ in the cleaning step.
Otherwise, if $\depth_{F^{\psol'}}(v) < \depthcap_\psol(w)$ then
either $w \notin \VtxFree^{\psol'}$ or $\depthcap_{\psol'}(w) > \depthcap_{\psol}(w)$.
We infer that, for every $P \in \Bb^{G[D]}_{u_1,u_2}$ such that $V(P) \cap N[v] \neq \emptyset$,
$\bucketmeasure^{\psol',D'}(\{u_1,u_2\})$ drops by at least one as compared to 
$\bucketmeasure^{\psol,D}(\{u_1,u_2\})$.
That is
\begin{align*}
\bucketmeasure^{\psol,D}(\{u_1,u_2\}) - \bucketmeasure^{\psol',D'}(\{u_1,u_2\})
 &\geq |\{P \in \Bb^{G[D]}_{u_1,u_2}~|~V(P) \cap N[v] \neq \emptyset\}| \\
 & \geq \frac{1}{2t} |\Bb^{G[D]}_{u_1,u_2}| \\
 & \geq \frac{1}{2t} \cdot \frac{1}{(t-1)(d+1)} \cdot \bucketmeasure^{\psol,D}(\{u_1,u_2\}).
\end{align*}
Furthermore, for every $\{u_1,u_2\} \in K \setminus \binom{D'}{2}$, the pair
$\{u_1,u_2\}$ no longer appears in the summation for $\measure(\psol',D')$. 
Hence for some universal constant $c$ (and since $|D| > 1$), 
  $$\measure(\psol,D) - \measure(\psol',D') \geq \frac{1}{2t} \binom{|D|}{2} \cdot \log_2 \frac{1}{1-\frac{1}{2t(t-1)(d+1)}} \geq \frac{c}{t^3(d+1)}|D|^2.$$
This completes the proof of the lemma.
\end{proof}


